Hierarchical Graph Network for Multi-hop Question Answering

In this paper, we present Hierarchical Graph Network (HGN) for multi-hop question answering. To aggregate clues from scattered texts across multiple paragraphs, a hierarchical graph is created by constructing nodes on different levels of granularity (questions, paragraphs, sentences, entities), the representations of which are initialized with pre-trained contextual encoders. Given this hierarchical graph, the initial node representations are updated through graph propagation, and multi-hop reasoning is performed via traversing through the graph edges for each subsequent sub-task (e.g., paragraph selection, supporting facts extraction, answer prediction). By weaving heterogeneous nodes into an integral unified graph, this hierarchical differentiation of node granularity enables HGN to support different question answering sub-tasks simultaneously. Experiments on the HotpotQA benchmark demonstrate that the proposed model achieves new state of the art, outperforming existing multi-hop QA approaches.

==> tables/exp_loss.tex <==
\begin{comment}
\paragraph{Effectiveness of Multi-task Loss}

As described in Section \ref{sec:prediction}, different node representations are utilized for different sub-tasks. Table \ref{table:HGN-loss} shows the ablation study results on paragraph selection loss $\mathcal{L}_{para}$ and entity prediction loss $\mathcal{L}_{entity}$. The span extraction loss $\mathcal{L}_{span}$ and supporting facts prediction loss $\mathcal{L}_{sent}$ are not ablated, since they are the essential final sub-tasks on which we evaluate the model. Using paragraph selection and entity prediction loss can further improve the joint F1 by 0.29 points, which demonstrates the effectiveness of optimizing all the losses jointly.
\begin{table}[t!]
%\small
\centering
\begin{adjustbox}{scale=0.95,center}
\begin{tabular}{lccc}
\hline
Objective & Ans F1 & Sup F1  & Joint F1 \\ \hline
$\mathcal{L}_{joint}$ &  \textbf{82.22} & \textbf{88.58} & \textbf{74.37} \\
-- $\mathcal{L}_{entity}$  & 82.16  & 88.49  & 74.23 \\
-- $\mathcal{L}_{para}$  & 81.92 & 88.25 & 73.76 \\
-- $\mathcal{L}_{entity}$ \& $\mathcal{L}_{para}$ &  82.26 & 88.30 & 74.08 \\ \hline
\end{tabular}
\end{adjustbox}
\caption{\label{table:HGN-loss}Ablation study on the proposed multi-task loss. RoBERTa-large is used for context encoding.}
\vspace{-3mm}
\end{table}
\end{comment}
